Monoidal strengthening of simple $\mathcal{V}$-polyhedral disjunctive cuts

Disjunctive cutting planes can tighten a relaxation of a mixed-integer linear program. Traditionally, such cuts are obtained by solving a higher-dimensional linear program, whose additional variables cause the procedure to be computationally prohibitive. Adopting a $\mathcal{V}$-polyhedral perspective is a practical alternative that enables the separation of disjunctive cuts via a linear program with only as many variables as the original problem. The drawback is that the classical approach of monoidal strengthening cannot be directly employed without the values of the extra variables appearing in the extended formulation. We derive how to compute these values from a solution to the linear program generating $\mathcal{V}$-polyhedral disjunctive cuts. We then present computational experiments with monoidal strengthening of cuts from disjunctions with as many as 64 terms. Some instances are dramatically impacted, with strengthening increasing the gap closed by the cuts from 0 to 100%. However, for larger disjunctions, monoidal strengthening appears to be less effective, for which we identify a potential cause.

==> defs.tex <==
\providecommand{\bibDirName}{include}  % *Modification: define file location
\providecommand{\parentDir}{.}  % *Modification: define file location
\providecommand{\mainDir}{.}  % *Modification: define file location
\providecommand{\includeDirName}{include}  % *Modification: define file location

\newcommand{\tableDir}{\mainDir/tables/}
\newcommand{\figDir}{\mainDir/figs/}

\newcommand{\biblio}{\bibliographystyle{include/splncs04}\bibliography{\mainDir/\bibDirName/akazachk}}  % *Modification: added 
%\newcommand{\biblio}{\printbibliography} % for biblatex

%== Other  =================================================

\newcommand{\rlaptext}[1]{\rlap{\text{#1}}}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%== Tikz  ==================================================

\newcommand{\xangle}{-20}
\newcommand{\yangle}{45}
\newcommand{\zangle}{90}

\newcommand{\xlength}{1}
\newcommand{\ylength}{1}
\newcommand{\zlength}{1}

\pgfmathsetmacro{\xx}{\xlength*cos(\xangle)}
\pgfmathsetmacro{\xy}{\xlength*sin(\xangle)}
\pgfmathsetmacro{\yx}{\ylength*cos(\yangle)}
\pgfmathsetmacro{\yy}{\ylength*sin(\yangle)}
\pgfmathsetmacro{\zx}{\zlength*cos(\zangle)}
\pgfmathsetmacro{\zy}{\zlength*sin(\zangle)}

\newcommand{\xX}{\xx}
\newcommand{\xY}{\xy}
\newcommand{\yX}{\yx}
\newcommand{\yY}{\yy}
\newcommand{\zX}{\zx}
\newcommand{\zY}{\zy}

%== Algorithms  ============================================

\RequirePackage{algorithmicx}
%\makeatletter
%\newcounter{algorithmicH}% New algorithmic-like hyperref counter
%\let\oldalgorithmic\algorithmic
%\renewcommand{\algorithmic}{%
%  \stepcounter{algorithmicH}% Step counter
%  \oldalgorithmic}% Do what was always done with algorithmic environment
%\renewcommand{\theHALG@line}{ALG@line.\thealgorithmicH.\arabic{ALG@line}}
%\makeatother
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\algnewcommand\algorithmicinit{\textbf{Initialize:}}
\algnewcommand\Initialize{\item[\algorithmicinit]}
\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]}
\algnewcommand\algorithmicpreprocessing{\textbf{Preprocessing:}}
\algnewcommand\Preprocessing{\item[\algorithmicpreprocessing]}
\newenvironment{varalgorithm}[1]
  {\algorithm\renewcommand{\thealgorithm}{#1}}
  {\endalgorithm}

\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  {{\parfillskip0pt\par}}\OldStatex\hskip\dimexpr#1\@tempdima\relax}
\makeatother

%== Text mode  =============================================

% complexity class
\newcommand{\complexity}[1]{\ensuremath{\mathcal{#1}}}

%% problem such as Max-Cut (conflicts with informs style)
%\newcommand{\problem}[1]{\textsc{#1}}

%== Custom math commands  ==================================

% "such that" such as used in the definition of a set
%\newcommand{\suchthat}{\mid}
\newcommand{\suchthat}{: }
%\newcommand{\suchthat}{\ \vert\ }

% "given" such as used in conditional probabilities and expectations
\newcommand{\given}{\nonscript\;\middle|\nonscript\;}

% indicator function (1 if true; 0 if false)
\newcommand{\indicator}[1]{\mathbf{1}\left[ #1\right]}

% definition of variable
%\newcommand{\defas}{\vcentcolon=} % vcentcolon needs mathtools
\newcommand{\defas}{:=}
\newcommand{\defeq}{\defas}
\newcommand{\eqdef}{=:}

\DeclareMathOperator{\bigO}{\mathcal{O}} % big O(micron)
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\cone}{cone}
\DeclareMathOperator*{\rec}{rec}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\relbd}{relbd}
\DeclareMathOperator*{\bd}{bd}
\DeclareMathOperator*{\cl}{cl}
\DeclareMathOperator*{\proj}{proj}
\DeclareMathOperator*{\err}{err}
\DeclareMathOperator*{\score}{sc}
\DeclareMathOperator*{\poly}{poly}
\newcommand{\jhat}{\hat\jmath}

% Linear algebra stuff
\DeclareMathOperator*{\cspan}{span}
\DeclareMathOperator*{\rspan}{rowspan}
\DeclareMathOperator*{\rank}{rank}
% \DeclareMathOperator*{\ker}{ker}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\ind}{\mathbbm{1}}
\renewcommand\vec{\mathbf}

%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} % abs, if mathtools is used
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\bigabs}[1]{\left\lvert#1\right\rvert}
\newcommand{\card}[1]{\lvert #1 \rvert}
\newcommand{\cardinality}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\bignorm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\innerprod}[1]{\langle #1 \rangle}
\newcommand{\bigmid}{\,\middle|\,}

\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\polar}{^{\circ}}
\newcommand{\reversepolar}{^{-}}

% scientific notation, 1\e{9} will print as 1x10^9
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}

% number systems
\newcommand{\field}[1]{\mathbbm{#1}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\posreals}{\reals_{>0}}
\newcommand{\nonnegreals}{\reals_{\ge 0}}
\newcommand{\posintegers}{\integers_{>0}}
\newcommand{\nonnegintegers}{\integers_{\ge 0}}
\newcommand{\posrationals}{\rationals_{>0}}
\newcommand{\nonnegrationals}{\rationals_{\ge 0}}
\newcommand{\R}{\reals}
\newcommand{\Rplus}{\nonnegreals}
\newcommand{\Rplusplus}{\posreals}
\newcommand{\C}{\field{C}}
\newcommand{\N}{\field{N}}
\newcommand{\Z}{\integers}
\newcommand{\Zplus}{\nonnegintegers}
\newcommand{\Zplusplus}{\posintegers}
\newcommand{\F}{\field{F}}
\newcommand{\Q}{\rationals}
%\newcommand{\E}{\mathbbm{E}}

%\newcommand{\Var}{\operatorname{Var}}
%\newcommand{\Cov}[1]{\text{Cov}\left[ #1 \right]}
%\newcommand{\E}{\mathbbm{E}}
%\newcommand{\rv}[1]{\boldsymbol{#1}}

\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\E}{\mathop{\bf E\/}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\Var}{\mathop{\bf Var\/}}
\newcommand{\Cov}{\mathop{\bf Cov\/}}
\newcommand{\stddev}{\mathop{\bf stddev\/}}

% short forms
\newcommand{\eps}{\epsilon}
\newcommand{\lam}{\lambda}
\newcommand{\vphi}{\varphi}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
%\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ol}[1]{\overline{#1}}

% calligraphic letters
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand\T{{\mathpalette\raiseT\intercal}} % custom transpose operator
\newcommand\raiseT[2]{\raisebox{0.25ex}{$#1#2$}}
\newcommand{\phT}{{\vphantom{\T}}} % vphantom to adjust subscript due to transpose operator

%% C plus plus
\usepackage{relsize}
%c from texinfo.tex
\def\ifmonospace{\ifdim\fontdimen3\font=0pt }

\newcommand{\Iff}{if\textcompwordmark f\xspace} % if and only iff

\def\Cpp{%
\ifmonospace%
    C++%
\else%
    %C\kern-.1667em\raise.30ex\hbox{\smaller{++}}%
    C\nolinebreak[4]\raisebox{0.5ex}{\tiny\textbf{++}}%
\fi%
\spacefactor1000 }

%== Cross-project definitions  =============================

\newcommand{\Clp}{\texttt{Clp}}
\newcommand{\Cplex}{\texttt{CPLEX}}
\newcommand{\Gurobi}{\texttt{Gurobi}}

\newcommand\basicvars{\mathcal{B}}
\newcommand\NB{\mathcal{N}}
\DeclareMathOperator{\vertices}{vert}
\newcommand{\pointset}{\mathcal{P}}
\newcommand{\rayset}{\mathcal{R}}
\newcommand{\CutLP}{CutLP}

\newcommand{\opt}[1]{\bar{#1}}
\newcommand{\lpopt}{\opt x}

\newcommand{\facetindex}[1]{^{#1}}
\newcommand{\initfacetindex}[1]{\init\facetindex{#1}}
\newcommand{\splitindex}[1]{_{#1}}

\newcommand{\Pindex}[1]{P\splitindex{#1}}
\newcommand{\Sindex}[1]{S\splitindex{#1}}
\newcommand{\Pk}{\Pindex{k}}
\newcommand{\Sk}{\Sindex{k}}

\newcommand{\onfloor}{\facetindex{1}}
\newcommand{\onceil}{\facetindex{2}}
\newcommand{\floorpointset}{\pointset\onfloor}
\newcommand{\ceilpointset}{\pointset\onceil}
\newcommand{\floorrayset}{\rayset\onfloor}
\newcommand{\ceilrayset}{\rayset\onceil}

%\newcommand{\intvars}{I}
\newcommand{\intvars}{\mathcal{I}}
%\newcommand{\PI}{P_{\intvars}}
\newcommand{\PI}{P_{I}}
\newcommand{\OPTCuts}{z'}
\newcommand{\OPTLP}{z_{\mathrm{LP}}}
\newcommand{\OPTIP}{z_{\mathrm{IP}}}
\DeclareMathOperator{\GAP}{\%\ gap\ closed}
\newcommand\LB{\mathit{LB}}
\newcommand\UB{\mathit{UB}}

%== Theorems  ==============================================
\ifspringer
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{observation}[theorem]{Observation}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{conjecture}[theorem]{Conjecture}
%
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{corollary*}{Corollary}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{proposition*}{Proposition}
%\newtheorem*{claim*}{Claim}
%\newtheorem*{example*}{Example}
%\newtheorem*{remark*}{Remark}
%\newtheorem*{observation*}{Observation}
%\newtheorem*{definition*}{Definition}
%\newtheorem*{conjecture*}{Conjecture}
\else
\newtheorem{theorem}{Theorem}

%% Everything below will be numbered sequentially
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newtheorem{thm}[theorem]{Theorem}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{obs}[theorem]{Observation}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{conj}[theorem]{Conjecture}
\fi

==> vpc-defs.tex <==
\newcommand{\rlaptext}[1]{\rlap{\text{#1}}}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\newcommand\basicvars{\mathcal{B}}
\newcommand\NB{\mathcal{N}}
\DeclareMathOperator{\vertices}{vert}
\newcommand{\pointset}{\mathcal{P}}
\newcommand{\rayset}{\mathcal{R}}
\newcommand{\opt}[1]{\bar{#1}}
\newcommand{\lpopt}{\opt x}
\newcommand{\intvars}{\mathcal{I}}
%\newcommand{\PI}{P_{\intvars}}
\newcommand{\PI}{P_{I}}

% \newcommand{\epsortho}{\epsilon_{\text{orth}}}
% \def\PRLPeq{PRLP\textsuperscript{=}}
% % \newcommand{\finalpointset}{{\pointset}_{*}}
% % \newcommand{\finalrayset}{{\rayset}_{*}}
% %\newcommand{\finalpointset}{\overset{*}{\pointset}\vphantom{\pointset}}
% %\newcommand{\finalrayset}{\overset{*}{\rayset}\vphantom{\pointset}}

% \newcommand{\nbspace}[1]{\tilde{#1}}
% \newcommand{\typeL}{\raisebox{\depth}{\small<}}
% \newcommand{\typeG}{\raisebox{\depth}{\small>}}
% \newcommand{\typeE}{\raisebox{\depth}{\small=}}
